Liquid Democracy: An Analysis in Binary Aggregation and Diffusion

The paper proposes an analysis of liquid democracy (or, delegable proxy voting) from the perspective of binary aggregation and of binary diffusion models. We show how liquid democracy on binary issues can be embedded into the framework of binary aggregation with abstentions, enabling the transfer of known results about the latter---such as impossibility theorems---to the former. This embedding also sheds light on the relation between delegation cycles in liquid democracy and the probability of collective abstentions, as well as the issue of individual rationality in a delegable proxy voting setting. We then show how liquid democracy on binary issues can be modeled and analyzed also as a specific process of dynamics of binary opinions on networks. These processes---called Boolean DeGroot processes---are a special case of the DeGroot stochastic model of opinion diffusion. We establish the convergence conditions of such processes and show they provide some novel insights on how the effects of delegation cycles and individual rationality could be mitigated within liquid democracy. The study is a first attempt to provide theoretical foundations to the delgable proxy features of the liquid democracy voting system. Our analysis suggests recommendations on how the system may be modified to make it more resilient with respect to the handling of delegation cycles and of inconsistent majorities.

==> Stuffwecut.tex <==
\subsection{old version of thm 1 and corollaries}

%%%%%%%%%%%%%%%%%OLD VERSION BELOW
\begin{theorem}\label{thm:quotarules}
Let $\S$ be a BA structure. 
An aggregator $F: (\AB_{c})^\N \to \AB$ is a quota rule if and only if it is anonymous, independent, monotonic, and responsive. 
%non-useless
\end{theorem}

\begin{proof}
\fbox{Left-to-right} Easily checked.
\fbox{Right-to-left} Let $\S$ be a BA structure. Let $F$ be an anonymous, independent, monotonic, and responsive aggregator. 

By \textit{anonymity} and \textit{independence}, for any $p\in\Atoms$, and any $\O\in\AB$, the only information determining $F(O)(p)$ is $|\O(p)|$ and $|\O(p^-)|$. 
%\item  by non-uselessness it is not the case that for all profiles $\O\in\AB$, $F(\O)(p)=*\}$. We proceed by case distinction:

By \textit{responsiveness}, there exists a non-empty set of profiles $S^\1=\{\O\in\AB|F(\O)(p)=\1\}$. Pick $\O$ to be any profile in $S^\1$ with the minimal value of $\frac{|\O(p)|}{|\O(p^\pm)|}$ and call this value $q_\1$. Now let $\O'$ be any profile such that $\O'=_{-i}\O$ and $\frac{|\O'(p)|}{|\O'(p^\pm)|}>q_\1$. This implies that 
either $O_i(p)\neq \1$ and $O'_i(p)=\1$, or $O_i(p)=\0$ and $O'_i(p)\neq \0$. In both cases, by \textit{monotonicity}, $F(\O')(p)= \1$. 
By iterating this reasoning on monotonicity and by anonimity, we can generate similarly any profile $\O$ such that $\frac{|\O(p)|}{|\O(p^\pm)|}>q_\1$, and show that $F(\O)(p)=\1$. Given that $q_\1$ was defined as a minimum, we conclude that for all $\O\in\AB$, $F(\O)(p)=1$ iff $\frac{\O'(p)}{\O'(p^\pm)}\geq q_\1$.

%THAT WAS THE PART TO FIND THE ABSOLUTE QUOTA, ASSUMING WE DON'T START WITH A GIVEN NUMBER OF AGENTS: Fix $q_1$ to be the value such that for any aggregation structure $\S$ and any profile $\O$ in $\AB$: $\frac{|\O(p)|-1}{|\O(p^\pm)|}< q_\1 < q \in $: $F(\O)(p)=\1$ iff $\frac{|\O'(p)|}{|\O'(p^\pm|)}> q_\1$.  

By \textit{responsiveness} again, there also exists a non-empty set of profiles $S^\0$ such that $S^\0=\{\O\in\AB|F(\O)(p)=\0\}$. Take $\O$ to be one of the profiles in $S^\0$ with minimal value of $\frac{|\O(p^-)|}{|\O(p^\pm)|}$ and let us call this value $q_\0$. By \textit{monotonicity} and the same reasoning steps as above, we obtain that for any profile $\O$ in $\AB$: $F(\O)(p)=\0$ iff $\frac{|\O(p^-)|}{|\O(p^\pm|)}\geq q_\0$. 



\begin{comment}
By responsiveness, there exists a set of profiles $S$ such that $S=\{\O\in\AB|F(\O)(p)=\0\}$. Take $\O$ to be a profile in $S$ with the minimal value of $q$ with $q=\frac{|\O(p^-)|}{|\O(p^\pm)|}$. 

Let $\O'\in\AB$ be such that $\O'=_{-i}\O$ and $\frac{|\O'(p^-)|}{|\O'(p^\pm)|}>q$. This implies that 
either $O_i(p)\neq \0$ and $O'_i(p)=\0$, or $O_i(p)=\1$ and $O'_i(p)\neq \1$. In both cases, by monotonicity, $F(\O')(p)= \0$.
By iterating this reasoning on monotonicity and by anonimity, we can treat in a similar way all profiles such that $\frac{|\O(p^-)|}{|\O(p^\pm)|}>q$, and show that $F\O=\0$. Given that $q$ was chosen to be minimal, we conclude that for all $\O\in\AB$, $F(\O)(p)=\0$ iff $\frac{\O'(p^-)}{\O'(p^\pm)}\geq q$.

Fix $q_-$ be the value such that for any aggregation structure $\S$ and any profiles $\O$ in $\AB$: $\frac{|\O(p^-)|-1}{|\O(p^\pm)|}< q_- < q \in $: $F(\O)(p)=\0$ iff $\frac{|\O'(p^-)|}{|\O'(p^\pm|)}> q_-$.
\end{comment}

\end{proof}

\begin{fact}\label{fact:symm}
Let $\S$ be a BA structure.
Let $F$ be a quota rule. $F$ is symmetric if and only if it is unbiased.
%\footnote{May's theorem relies on the additional assumption that the number of agents is odd. We do not need this assumption, given that our majority rule is defined to be unbiased for any number of agents.}
\end{fact}
\begin{proof}
This follows from the definitions of symmetric quotas and of unbiasedness. Let $F$ be a quota rule. The following statements are all equivalent: 
\begin{enumerate}
\item $F$ is unbiased (assumption); 
\item For all $\O,\O'$ in $\AB$ such that, for all $i\in\N, O_i(p)=\1$ iff $O'_i(p)=\0$,  $|O(p)|>p_\1$ iff $|O'(\neg p)|>p_\0$ (definition of unbiasedness)
\item $q_\1=q_\0$ (definition of quota rule)
\item $F$ is symmetric (definition of symmetric quota rule). 
\end{enumerate}
This completes the proof.
\end{proof}

\begin{corollary}\label{thm:MayAdaptedNEW}
%Let $\S$ be a BA structure. 
%where $\gamma$ is simple.
%and $|\N|$ is odd. WE DON'T NEED THIS CONDITION ANYMORE
Let $\S$ be a BA structure. An aggregator $F$ is a symmetric quota rule if and only if it is independent, anonymous, monotonic, responsive, and unbiased. 
%\footnote{May's theorem relies on the additional assumption that the number of agents is odd. We do not need this assumption, given that our majority rule is defined to be unbiased for any number of agents.}
\end{corollary}
\begin{proof}
This follows directly from Theorem \ref{thm:quotarules} and Fact \ref{fact:symm}.
%Let $F$ be an aggregator.By the previous lemma, $F$ is monotonic, anonymous, and responsive iff it is a quota rule, and by the previous fact, $F$ is a symmetric quota rule iff it is unbiased.
\end{proof}

%\textcolor{blue}{I think the proof is already there. Notice that RAT is used in the book in the step where you, by exclusion, conclude in step (ii) that the value must me $\0$ or $\ast$ (you are simply using here the type of the aggregator, that is that the codomain must be a partial valuation, instead of RAT). Now for the last case. Suppose the value is $\ast$, then by monotonicity (check the definition we give of montonicity as it should match!) it should remain $\ast$ as the number of $\1$s grows. By unbiasedness the same should happen with the $\0$s, and therefore the aggregator would always output $\ast$, against the assumption of responsiveness. QED}

\begin{corollary}
An aggregator $F$ is the majority aggregator $\maj$ if and only if it is an anonymous, independent, monotonic, responsive, and unbiased aggregator which minimizes abstention. 
\end{corollary}
\begin{proof}
\ldots 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{the proxy majority without abstention}
The standard form of proxy voting can be modeled by the following proxy aggregator based on issuewise majority:

\begin{align}
\pv_{\maj}(\O)(p) = 1 & \IFF \sum_{i \in \O(p)} w^\O_i(p) \geq \frac{|\N|+1}{2} \label{eq:proxymaj}
\end{align}

That is, an issue is accepted by proxy majority in profile $\O$ if and only if the sum of the weights of the agents who accept $p$ in $\O$ exceeds the majority quota. Just like majority, proxy majority is not collectively consistent. In general, given an (anonymous and independent) aggregator $F$, its proxy variant can be defined as in \eqref{eq:proxymajast} for $\maj$.

Remark that the notation introduced above allows us to define the majority rule without abstention $\maj$ in a simpler way:

\begin{align}
\pv_{\maj}(\O)(p) = 1 & \IFF |\{i \in \N | O_{g_i}(p)=\1 \}| \geq \frac{|\N |+1}{2} \label{eq:proxymajsimple}
\end{align}

\subsection{Our initial axiomatic properties for proxy aggregators}

We start by defining proxy variants of well-known properties of aggregators from the judgment aggregation literature. Let us first, however, introduce some auxiliary notation and terminology. 

We start by defining a notion of opinion permutation for proxy profile. Indeed, the permutation of a proxy profile cannot simply be defined by `reshuffling' the individual proxy opinions in the profile. 
%\footnote{The permutation of a proxy profile cannot simply be defined by `reshuffling' the individual proxy opinions in the profileIf $i$ delegates to $j$, and the permutation $\mu$ is such that $i \mapsto k$ and $j \mapsto \ell$ (with $i \neq j \neq k \neq \ell$), then $k$'s opinion in the permuted profile should be a delegation to $\ell$ rather than to $j$.THAT'S NOT ENOUGH}
We therefore introduce a notion of issue by issue opinions permutation which is relative to connected components of the delegation graphs and preserve the rationality of the individual opinions, i.e an agent $i$ may switch opinions on two different issues $p$ and $q$  with two different agents $j$ and $k$ respectively, as long as: 1) there is a path between $i$ and $j$ in the delegation graph $G_p$ and a path between $i$ and $k$ in the delegation graph $G_q$, and 2) the resulting profile satisfies the individual rationality constraint.

\begin{definition}[issuewise connectedness preserving permutation]
Given an issue $p\in P$, a $p$-connectedness preserving permutation is a bijection $\mu_p: \N\rightarrow\N$, such that, for all $i\in\N$, $iR^*_{p}\mu_p(i)$ or $\mu_p(i)R^*_pi$.
\end{definition}

\begin{definition}[rational proxy permutation]
Given a proxy profile $\O$, a rational proxy opinions permutation $\mu:\mathcal{P}^\N\to\mathcal{P}^\N$ is a function where  $\mu(\O) = \tuple{O^\mu_1, \ldots, O^\mu_n}$ is such that, for all $i\in\N$, and all $p\in\Atoms$:
\begin{description}
\item $O^\mu_i(p) =  O_{\mu_p(i)}(p)$,
\item $\mu_p$ is a $p$-connectedness preserving permutation, and
\item $O^\mu_i$ satisfies the formulas in \eqref{eq:ir}.
\end{description}
\end{definition}

%HERE IS THE NEW (``SLIGHTLY LESS AD HOC") DEFINITION: We define a notion of permutation relative to connected components of a delegation graph, i.e only agents between which a path exists are permuted. \begin{definition}[connectedness preserving permutation] Given a proxy profile $\O$ and an issue $p\in P$, a \emph{connectedness preserving permutation} is a bijection $\mu: \N\rightarrow\N$, such that, for all $i\in\N$, $iR^*_{p}\mu(i)$ or $\mu(i)R^*_pi$.\end{definition}

%\begin{definition}[permutation OLD DEFINITION]OLD (SUPER AD HOC) DEFINITION: Given a bijection $\mu: \N\rightarrow\N$, and a proxy profile $\O$, we denote with $\O^\mu = \tuple{O^\mu_1, \ldots, O^\mu_n}$ the permutation of $\O$ where:$O^\mu_i(p) = \left\{ \begin{array}{ll} \O_{i}(p) & \mbox{if $i$ is a guru for $p$ in $\O$} \\ \mu(j) & \mbox{if $iR_pj$ in $\O$} \end{array} \right.$ \end{definition}THIS TYPE OF PERMUTATION KEEPS THE NETWORKS ISOMORPHIC (AND WITH THE SAME OPINION FOR THE CORRESPONDING GURUS). WE WANT SOMETHING MORE GENERAL: THERE SHOULD BE ANOTHER TYPE OF TRANSFORMATION OF OUR PROFILE WHICH ONLY PRESERVES THE NUMBER OF AGENTS WHO ADD WEIGHT TO OPINION 1 AND WHO ADD WEIGHT TO OPINION ZERO. THAT IS, WE ONLY NEED TO PRESERVE THE CARDINALITIES OF THE SETS OF ALL AGENTS WITH GURUS WITH OPINION $\0$ AND WITH OPINION $\1$. THAT WOULD DEFINE THE SET OF PROXY PROFILES WHICH TRANSLATE TO THE SAME NON-PROXY PROFILE WITH ABSTENTION. BUT THEN IT IS NOT JUST A SIMPLE "PERMUTATION" ANYMORE.    

\begin{definition}
A proxy aggregator $\pv:\mathcal{P}^\N \to \AB$ is said to be:
\begin{description}
\item[unanymous] iff for all $p\in \Atoms$, for all proxy profile $\O$ : if for all $i\in \N$, and all $x \in \{\0,\1\}$, $O_{g_p(i)}(p) = x$, then $\pv(\O)(p)=x$ and if for all $i\in \N$, $g_p(i)=\emptyset$, then $\pv(\O)(p)=\ast $. I.e., when all gurus agree, their opinion on an issue becomes the group's opinion on it, and when there are no gurus for this issue, the group abstains on it. 
%\item[unanymous bis] iff for all $p\in \Atoms$, for all proxy profiles $\O$: if for all $i\in \N, O_i(p) = \1$, then $\pv(\O)(p)= \1$ and if for all $i\in \N, O_i(p) \neq \1$, then $\pv(\O)(p)\neq \1$. 
\item[anonymous] iff for any rational proxy permutation $\mu: \mathcal{P}^\N\rightarrow\mathcal{P}^\N$, $\pv(\O)=\pv(\O^\mu)$. I.e., rationally permuting proxy opinions among individuals does not affect the output of the aggregator.

\item[$p$-dictatorial] iff there exists $i \in \N$ (the {\em $p$-dictator}) s.t. for any proxy profile $\O$, and all $x \in \set{\0,\1}$, $\pv(\O)(p)= x$ iff  $g_p(i) \neq \emptyset$ and $\O_{g_p(i)}  = x$ . 
I.e., there exists an agent whose guru's opinion always determines the group's opinion on $p$. If the aggregator is $p$-dictatorial, with the same dictator on all issues $p \in \I$, then it is called {\bf dictatorial}.
%\item[$p$-dictatorial bis] iff there exists $i \in \N$ (the {\em $p$-dictator}) s.t. for any proxy profile $\O$, $\pv(\O)(p) = \O_i(p)$. I.e., there exists an agent whose opinion always determines the group's opinion on $p$. If the aggregator is $p$-dictatorial, with the same dictator on all issues $p \in \I$, then it is called {\bf dictatorial}.

\item[$p$-oligarchic] iff there exists $C \subseteq \N$ (the {\em $p$-oligarchs}) s.t. $C\neq\emptyset$ and for any proxy profile $\O$  and any value $x \in \set{\0,\1}$: $\pv(\O)(p) = x $ iff for all $i\in C$ , $g_p(i)\neq\emptyset$ and $O_{g_p(i)}=x$. I.e., there exists a group of agents whose gurus' opinion always determines the group's opinion on $p$. If the aggregator is $p$-oligarchic, with the same oligarchs on all issues $p \in \Atoms$, then it is called {\bf oligarchic}.
%\item[$p$-oligarchic bis] iff there exists $S \subseteq \N$ (the {\em $p$-oligarchs}) s.t. $S\neq\emptyset$ and for any proxy profile $\O$, $\pv(\O)(p) = \1$ if and only if, for all $i\in S$, $O_i(p)=\1$. I.e., there exists a group of agents whose opinion always determines the group's opinion on $p$. If the aggregator is $p$-oligarchic, with the same oligarchs on all issues $p \in \I$, then it is called {\bf oligarchic}.
\item[monotonic] iff, for all $p\in \Atoms$ and all $i\in\N$: for any proxy profiles $\O, \O'$, if $\O =_{-i} \O'$ and $O_i(p)\neq 1$ and $O'_i(p)=1$, then: if $\pv(\O)(p)=1$, then $\pv(\O')(p)=1$.
%\item[monotonic bis?] iff, for all $p\in \Atoms$ and all $i\in\N$: for any proxy profiles $\O, \O'$, if $\O =_{-i} \O'$ and $O_i(p)\neq 1$ and $O'_i(p)=1$, then: if $\pv(\O)(p)=1$, then $\pv(\O')(p)=1$.

\item[independent] iff, for all $p\in \Atoms$, for any proxy profiles $\O, \O'$: if for all $i\in \N, O_{g_p(i)}(p) = O'_{g'_p(i)}(p)$, then $\pv(\O)(p)=\pv(\O')(p)$.
%\item[independent bis] iff, for all $p\in \Atoms$, for any proxy profiles $\O, \O'$: if for all $i\in \N, O_i(p) = O'_i(p)$, then $\pv(\O)(p)=\pv(\O')(p)$.
\item[neutral] iff, for all $p,q \in \Atoms$, for any proxy profile $\O$: if for all $i\in\N$, $O_{g_p(i)}(p)=O_{g_q(i)}(q)$, then $\pv(\O)(p)=\pv(\O)(q)$.
%\item[neutral bis] iff, for all $p,q \in \Atoms$, for any proxy profile $\O$: if for all $i\in\N$, $O_i(p)=O_i(q)$, then $\pv(\O)(p)=\pv(\O)(q)$.
\item[systematic] iff it is neutral and independent.
\item[unbiased] iff for all $p \in \Atoms$, for any proxy profiles $\O, \O'$: if for all $i\in\N$, $O_{g_p(i)}(p)= \1$ iff $O'_{g_p(i)}(p)=\0$, then $\pv(\O)(p)=\1$ iff $\pv(\O')(p)=\0$. 
%\item[unbiased bis] iff for all $p \in \Atoms$, for any proxy profiles $\O, \O'$: if for all $i\in\N$, $O_i(p)= 1$ iff $O'_i(p)\neq \1$, then $\pv(\O)(p)=\1$ iff $\pv(\O')(p)\neq \1$. 
\item[collectively rational] iff for any proxy profile $\O$, $\pv(\O) \models \gamma$. I.e., if the aggregator preserves the constraint $\gamma$. 
\end{description}
\end{definition}
It is worth briefly commenting on the above definitions. Like in the classic case, anonymity implies non-dictatorship. A weaker form of dictatorship would require the opinion of the dictator to become the collective opinion only in those cases in which the dictator herself is a guru. This would be the case when one agent is a guru for more than half of the population. 



\section{To-do-list}

subsection{Properties on Network-Invariant Profiles}

Let us assume that we restrict the set of possible proxy profiles to the ones with the same delegation structures (with respect to each issue). In that case, proxy majority becomes $p$-oligarchic---the oligarchs being the set of gurus such that more than half of the voters is related to any of them via $R^*_p$. Proxy majority would be oligarchic only if there existed a unique group of agents such that, for each opinion profile, \emph{for any issue $p$}, they were "p-oligarchs", which is not the case.

%(and the rule becomes dictatorial whenever there is only one such agent).
However, if we restrict even more our set of possible opinion profiles to the ones with a unique fixed network (i.e., the same network for all issues), then proxy majority becomes oligarchic.

\ldots

\subsubsection{Oligarchy}
An aggregator is said to be \emph{oligarchic} if there exists a non-empty set of agents (the oligarchs) such that, for any opinion profile, an issue is collectively accepted if and only if it is accepted by all the oligarchs. Majority proxy voting is not oligarchic in general. 


\subsubsection{isomorphic networks}
Going towards the opposite direction, if we restrict our set of possible opinion profiles to the ones with isomorphic network structures (OR TO STRUCTURES WHICH ARE SIMILAR IN THE SENSE OF THE ABOVE AD HOC CONDITION), then we obtain a \emph{random issuewise oligarchy}. To make majority proxy voting properly oligarchic would require to add a stronger constraint to the set of opinion profiles: there is a unique set of agents such that for all opinion profiles, those agents are followed by more than half the population with respect to \emph{all} issues.  

\subsubsection{Standard impossibility results}

The above defined opinion profiles can be mapped into a (non-proxy) opinion profile with abstention, as follows: For any proxy opinion profile, any agent and any issue $p$, if the agent is related via $R^*_p$ to an agent with opinion $0$ or $1$, then this agent is assigned opinion $0$ (respectively $1$) on issue $p$, otherwise this agent is abstaining on $p$. 
 

Therefore, standard impossibility results for aggregation with abstention apply: every aggregation function that is independent and unanimous must be weakly oligarchic.

\subsection{Truth-tracking Behavior}

Condorcet's Jury Theorem shows that, for individuals whose probability of choosing the right alternative (among 2) is above 0.5, the probability of correct collective decision under the majority rule is (higher than the individual one and) approaches 1 as the size of the group increases.

When considering proxy voting, if we assume that all agents have the same probability of choosing correctly, then they would be better off without any delegation, as delegating reduces the number of impactful decision makers. 
To make delegation truth-tracking, one thus needs to assume that when agents choose to delegate, they do so rather wisely too: they have more chances to delegate to someone who chooses more accurately than themselves than not (i.e, there is a probability above 0,5 that their delegate has a higher probability of making the right choice than theirs).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}[Conjecture]
An independent aggregator $F: (\AB_{c})^\N \to \AB$ is anonymous if and only if the corresponding proxy aggregator $\pv_F:\mathcal{P}^\N \to \AB$ is. 
\end{theorem}
\begin{proof}
\begin{comment}
$\Leftarrow$:
Let $\pv_F:\mathcal{P}^\N \to \AB$ be an anonymous proxy aggregator.  
Then, for any rational proxy permutation $\nu: \mathcal{P}^\N\rightarrow\mathcal{P}^\N$, $\pv(\O)=\pv(\O^\mu)$, i.e., any function where  $\nu(\O) = \tuple{O^\nu_1, \ldots, O^\nu_n}$ is such that, for all $i\in\N$, and all $p\in\Atoms$: i) $O^\nu_i(p) =  O_{\nu_p(i)}(p)$, ii) $\nu_p$ is a $p$-connectedness preserving permutation (a bijection $\nu_p: \N\rightarrow\N$, such that, for all $i\in\N$, $iR^*_{p}\nu_p(i)$ or $\nu_p(i)R^*_pi$.) ; and iii) $O^\nu_i$ satisfies the formulas in \eqref{eq:ir}.

$\Rightarrow$:
Let $F: (\AB_{c})^\N \to \AB$ be an independent and anonymous aggregator. Then, for any bijection $\mu: \N\rightarrow\N$, $F(\O)=F(\O^\mu)$, where $\O^\mu = \tuple{O_{\mu(1)}, \ldots, O_{\mu(n)}}$. 

Proxy aggregator $\pv_F:\mathcal{P}^\N \to \AB$ is anonymous iff for any rational proxy permutation $\nu: \mathcal{P}^\N\rightarrow\mathcal{P}^\N$, $\pv(\O)=\pv(\O^\mu)$, i.e., any function where  $\nu(\O) = \tuple{O^\nu_1, \ldots, O^\nu_n}$ is such that, for all $i\in\N$, and all $p\in\Atoms$:
\begin{description}
\item $O^\nu_i(p) =  O_{\nu_p(i)}(p)$,
\item $\nu_p$ is a $p$-connectedness preserving permutation (a bijection $\nu_p: \N\rightarrow\N$, such that, for all $i\in\N$, $iR^*_{p}\nu_p(i)$ or $\nu_p(i)R^*_pi$.)
\item $O^\nu_i$ satisfies the formulas in \eqref{eq:ir}.
\end{description}
\end{comment}
\ldots
\end{proof}


\begin{theorem}[The case of the majority rule]
 Let ${\O}$ be a proxy profile, and $t$ be the above defined translation function from a proxy profile to an opinion profile. 
Then, $\pv_{\maj_\ast}(\O)=\maj_\ast(t(\O))$.
\end{theorem}

\begin{proof}
Let $p\in \Atoms$ be arbitrary, and $x\in\{0,1\}$. Then:
\begin{align*}
& \pv_{\maj_\ast}(\O)(p)=x & \mbox{ iff } \\ 
& |\{i \in \N | O_{g_p(i)}(p)=x\}| >  |\{i \in \N | O_{g_p(i)}(p)=(1-x)\}|& \mbox{ iff }  \\
& |\{i \in \N | t(O_i(p))= x \}| > |\{i \in \N | t(O_i(p))= (1-x)\}|& \mbox{ iff }  \\
& \maj_\ast(t(\O))(p)=x. & 
\end{align*}
And therefore:
\begin{align*}
\pv_{\maj_\ast}(\O)(p)=\ast \mbox { iff }  \pv_{\maj_\ast}(\O)(p)\notin \{0,1\} \mbox { iff } \\
 \maj_\ast(t(\O))(p) \notin \{0,1\}  \mbox { iff }  \maj_\ast(t(\O))(p) = \ast.\\
\end{align*}
\end{proof}

The same proof goes through when replacing $\frac{1}{2}$ by any other quota, showing that the correspondence holds for any similarly defined proxy quota rule. 

\begin{theorem}[The case of dictatorships]
Let ${\O}$ be a proxy profile, and $t$ be the above defined standard translation from a proxy profile to an opinion profile. Let $dic\ast$ be a dictatorial aggregator and $ \pv_{dic\ast}$ be a dictatorial proxy aggregator. 
Then, $\pv_{dic\ast}({\O})=dic\ast(t({\O}))$.
\end{theorem}
\begin{proof}
Let $p\in \Atoms$ be arbitrary, agent $i$ be a proxy dictator, and $x\in\{\0,\1\}$
\begin{align*}
 \pv_{dic_\ast}({\O})(p)=x &  \mbox{ iff} \\ 
O_{g_p(i)}(p)=x & \mbox{ iff}  \\
t(O_i(p))= x & \mbox{ iff} \\
 dic_\ast(t({\O}))(p)=x &
\end{align*}
And therefore:
\begin{align*}
\pv_{dic_\ast}(\O)(p)=\ast \mbox { iff }  \pv_{dic\ast}(\O)(p)\notin \{0,1\} \mbox { iff } \\
 dic_\ast(t(\O))(p) \notin \{0,1\} \mbox { iff }  dic_\ast(t(\O))(p) = \ast.\\
\end{align*}
\end{proof}


\subsection{Proxy Majority}
%Proxy majority is unanimous, anonymous\footnote{Note that this is the case in a very weak sense relying on our definition of rational permutations.}, monotonic, systematic, not rational (but $\gamma$-rational when $\gamma$ is simple), and unbiased.

Our variant of May's characterization theorem \cite{May_1952} of majority voting \ref{thm:MayAdapted} now applies to  proxy majority:

\begin{theorem}[Corollary]
Let $\S$ be a BA structure where $\gamma$ is simple. 
%and $|\N|$ is odd. WE DON'T NEED THIS CONDITION ANYMORE
A proxy aggregator $\pv$ is the proxy majority $\pv_{\maj_\ast}$ if and only if it is rational, monotonic, anonymous, responsive, and unbiased. TO BE CORRECTED.
\end{theorem}
\begin{proof}
This follows directly from Theorem \ref{thm:MayAdapted} STILL TO BE CORRECTED and Definition \ref{}. 
\end{proof}

\subsection{Impossibility in Proxy Voting}
We obtain the corresponding impossibility result (similarly as the result for binary judgment aggregation with abstention):

\begin{theorem}[proxy impossibility]
Let $\S$ be a BA structure such that the agenda induced by $\gamma$ is path connected and evenly negatable. 
Then if a proxy aggregator $\pv: \mathcal{P}^\N \to \AB$ is independent, unanimous and collectively rational, then it is oligarchic.
\end{theorem}


\begin{comment}
%%%%%THIS IS THE OLD PROOF (WITHOUT BOUND)
\begin{proof}
Assume that for all $p\in \Atoms$, for all $S\subseteq\N$ such that $S$ is a cycle in $G_{p}$, for all $i,j\in S$: $O_i(p)=O_j(p)$.
Consider an arbitrary $p\in \Atoms$, and an arbitrary $i\in \N$. Let $k$ be the distance from $i$ to $l$, where $l$ is the closest agent in a cycle $S\subseteq\N$ of $G_p$. We show that for any such $k\in\mathbb{N}$, there exists an $n \in \mathbb{N}$, such that $O^{n}_ i(p)$ is stable.
\begin{itemize}
\item If $k=0$: $i\in S$, hence $O_{i}(p)$ is stable. 
\item if $k=n+1$: Assume that for agent $j$ at distance $n$ from $l$, 
for some $m \in \mathbb{N}$, $O^{m}_ j(p)$ is stable. We need to consider the following cases:
\begin{enumerate}
\item If $\bigwedge_{p \in \Atoms} O^{m}_{R_p(i)}(p) \wedge \bigwedge_{\varphi \in \C}$ is consistent, 
then $O^{m+1}_i(p)=O^m_j(p)$, and $O^{m+1}_i(p)$ is stable. 
\item If $\bigwedge_{p \in \Atoms} O^{m}_{R_p(i)}(p) \wedge \bigwedge_{\varphi \in \C}$ is not consistent, then:
\begin{enumerate}
\item if $O^{m}_i(p)=O^m_j(p)$, then $O^{m}_i(p)$ is stable. 
\item if $O^{m}_i(p) \neq O^m_j(p)$, then:
%$\O^{m+1}_i(p) = \O^{m}_i(p)$: $i$ does not change his opinion at stage $m+1$ but this does not guarantee that this won't change later on:
\begin{enumerate}
\item If there is a $t\in\mathbb{N}$ such that $\bigwedge_{p \in \Atoms} O^{m+t}_{R_p(i)}(p) \wedge \bigwedge_{\varphi \in \C}$ is consistent, then $O^{m+t+1}_i(p) = O^{m}_j(p)$, and $O^{m+t+1}_i(p)$ is stable.
\item If there is no such $t$, then $i$'s opinion on $p$ will never change: $O^{m}_i(p)$ is stable. 
\end{enumerate}
\end{enumerate}
\end{enumerate}
\end{itemize}
\end{proof}
\end{comment}

\begin{comment} BELOW IS THE OLD DEFINITION, FOR MEMORY
\begin{definition}[Quota rules]
Let $\S$ be an aggregation structure. An aggregator $F:(\AB_{c})^\N \to \AB$ is a {\em quota rule} if there exist $q_\1, q_\0 \in \mathbb{Q}$ such that, for $x \in \set{\0, \1}$:
\begin{align}
0<q_x\leq 1 \label{eq:nontrivial}, \\ 
q_x > 1 - q_{(\1 - x)}, \label{eq:constraint}
\end{align}
and for any issue $p\in\Atoms$, and any opinion profile $\O\in\AB$:
\begin{align}\label{eq:quotarules}
F(\O)(p)=  
\begin{cases}
        \1  & \mbox{ if }  |\O(p)|  \geq  q_\1 |\O(\pm p)|\\
        \0  & \mbox{ if }  |\O(\neg p)| \geq q_\0 |\O(\pm p)|  \\
       \ast & \mbox{ otherwise }   \\
\end{cases}
\end{align} \label{eq:quota}
If $q_\1 = q_\0$ then the quota rule is called {\em symmetric}.
\end{definition}
\end{comment}

\begin{comment}below the very same steps of $q_\0$:
By responsiveness, there exists a set of profiles $S$ such that $S=\{\O\in\AB|F(\O)(p)=\0\}$. Take $\O$ to be a profile in $S$ with the minimal value of $q$ with $q=\frac{|\O(p^-)|}{|\O(p^\pm)|}$. 
Let $\O'\in\AB$ be such that $\O'=_{-i}\O$ and $\frac{|\O'(p^-)|}{|\O'(p^\pm)|}>q$. This implies that 
either $O_i(p)\neq \0$ and $O'_i(p)=\0$, or $O_i(p)=\1$ and $O'_i(p)\neq \1$. In both cases, by monotonicity, $F(\O')(p)= \0$.
By iterating this reasoning on monotonicity and by anonimity, we can treat in a similar way all profiles such that $\frac{|\O(p^-)|}{|\O(p^\pm)|}>q$, and show that $F\O=\0$. Given that $q$ was chosen to be minimal, we conclude that for all $\O\in\AB$, $F(\O)(p)=\0$ iff $\frac{\O'(p^-)}{\O'(p^\pm)}\geq q$.
Fix $q_-$ be the value such that for any aggregation structure $\S$ and any profiles $\O$ in $\AB$: $\frac{|\O(p^-)|-1}{|\O(p^\pm)|}< q_- < q \in $: $F(\O)(p)=\0$ iff $\frac{|\O'(p^-)|}{|\O'(p^\pm|)}> q_-$.
\end{comment}

Let $F$ be a quota rule. The following statements are equivalent: 
\begin{enumerate}
\item $F$ is unbiased. (assumption) 
\item For all $\O,\O'$ in $\AB$ such that, for all $i\in\N, O_i(p)=\1$ iff $O'_i(p)=\0$,  
$|O(p)|\geq \lceil q_\1 |\O(\pm p)| \rceil$ iff 
$|O'(\neg p)|\geq \lceil q_\0 |\O'(\pm p)| \rceil$. (definitions of unbiasedness and quota rules)
\item $\lceil q_\1 |\O(\pm p)| \rceil =  \lceil q_\0 |\O(\pm p)| \rceil $
%(definition of quota rule)
\item $F$ is symmetric. (definition of symmetric quota rule) 
\end{enumerate}
%This completes the proof.

%%%%%%%%%%%%%%%%%%%%%%%%%%%% majority characterization

%\fbox{In one go}
Assume $F$ is a uniform symmetric quota rule: for all $\O\in\AB$, $\lceil q_\1 |\O(\pm p)| \rceil =  \lceil q_\0 |\O(\pm p)| \rceil$. Assume that $q_\1\leq\frac{1}{2}$. Then, by constraint \eqref{eq:constraint} $q_\0 \geq \frac{1}{2}$ and $F$ is not symmetric. Contradiction. Hence, $q_\1>\frac{1}{2}$. And by the same reasoning, $q_\0>\frac{1}{2}$. Two cases: 
\begin{itemize}
\item[i] $F$ is not $\maj$: $q_\1, q_\0>\frac{1}{2}+\frac{1}{2|N|}$. 
Then $|\{\O\in\AB | F(\O)(p)= \1 \} \subset \{\O\in\AB | \maj(\O)(p)= \1 \}$ and $\{\O\in\AB | F(\O)(p)= \0 \} \subset \{\O\in\AB | \maj(\O)(p)= \0 \}$, therefore $\{\O\in\AB | F(\O)(p)= \ast \} \supset \{\O\in\AB | \maj(\O)(p)= \ast \}$. Therefore, $F$ does not minimize abstention. 

\item[ii] $F$ is $\maj$: $\frac{1}{2}<q_\1,q_\0 \leq \frac{1}{2}+\frac{1}{2|N|}$. Assume that for any symmetric quota rule $F'$ with quotas $\lceil q'_\1  |\O(\pm p)| \rceil =  \lceil q'_\0 |\O(\pm p)| \rceil $: $|\{\O\in\AB | F'(\O)(p)= \ast \}| \leq |\{\O\in\AB \mid \maj(\O)(p)=\ast \}|$. Then, by the above reasoning, we know that $\frac{1}{2}<q'_\1,q'_\0\leq \frac{1}{2}+\frac{1}{2|N|}$, and $F'$ is just $\maj$. Therefore, $F$ minimizes abstention.  
\end{itemize}
Hence, $F$ minimizes abstention iff $F$ is $\maj$.

\begin{comment}
\fbox{Left-to-right}
Assume $F$ is $\maj$.
Assume, for contradiction, that there exists a quota rule $F'$ with quotas $\lceil q'_\1 \times |\O(\pm p)| \rceil =  \lceil q'_\0 \times |\O(\pm p)| \rceil $  such that $|\{\O\in\AB | F'(\O)(p)= \ast \}| < |\{\O\in\AB \mid \maj(\O)(p)=\ast \}|$. Two cases:
\begin{itemize}
\item[i] $q_\1'\leq \frac{1}{2}$. Then by constraint  \eqref{eq:constraint}, $q'_\0 > \frac{1}{2}$, and $F'$ is not symmetric. Contradiction.
\item[ii] $q_\1'>\frac{1}{2}+\frac{1}{2|N|}$.  
Then $|\{\O\in\AB | F'(\O)(p)= \1 \} \subset \{\O\in\AB | \maj(\O)(p)= \1 \}$ and $\{\O\in\AB | F'(\O)(p)= \0 \} \subset \{\O\in\AB | F(\O)(p)= \0 \}$, therefore $\{\O\in\AB | F'(\O)(p)= \ast \} \supset \{\O\in\AB | \maj(\O)(p)= \ast \}$. Contradiction.\footnote{Another way to state this is: for all profiles $\O\in\AB$, if $F'(\O)(p)=\1$, then $\maj(\O)(p)=\1$, and if $F'(\O)(p)=\0$, then $\maj(\O)(p)=\0$, but  there exists some profiles where $p^\pm=N$ and $|O(p)|=\frac{1}{2}+\frac{1}{|N|}$, for which $\maj(\O)(p)=\1$ but $F'(\O)(p)=\ast$.}
\end{itemize}
Therefore, $\frac{1}{2}< q_\1', q_\0'\leq\frac{1}{2}+\frac{1}{2|N|}$, which implies that $F'(\O)(p)=\ast$ iff $\maj(\O)(p)=\ast$. Hence  $|\{\O\in\AB | F'(\O)(p)= \ast \}| = |\{\O\in\AB \mid \maj(\O)(p)=\ast \}|$. Contradiction. 

\fbox{Right-to-left}
Assume $F$ is a quota rule with $\lceil q_\1 \times |\O(\pm p)| \rceil =  \lceil q_\0 \times |\O(\pm p)| \rceil $ which minimizes abstention. Assume, for contradiction, that $F$ is not $\maj$. Two cases: 
\begin{itemize}
\item[i] $q_\1\leq\frac{1}{2}$. Then, by \eqref{eq:constraint} $q_\0 \geq \frac{1}{2}$ and $F$ is not symmetric.
Contradiction.
\item[ii] $q_\1>\frac{1}{2}+\frac{1}{2|N|}$. Then $|\{\O\in\AB | F(\O)(p)= \1 \} \subset \{\O\in\AB | \maj(\O)(p)= \1 \}$ and $\{\O\in\AB | F(\O)(p)= \0 \} \subset \{\O\in\AB | \maj(\O)(p)= \0 \}$, therefore $\{\O\in\AB | F(\O)(p)= \ast \} \supset \{\O\in\AB | \maj(\O)(p)= \ast \}$. Contradiction.
\end{itemize}
Hence, $\frac{1}{2}<q_\1=q_\0 \leq \frac{1}{2}+\frac{1}{2|N|}$. Therefore, $F$ is $\maj$.

\medskip

\fbox{In one go}
Assume $F$ is a symmetric quota rule: for all $\O\in\AB$, $\lceil q_\1 \times |\O(\pm p)| \rceil =  \lceil q_\0 \times |\O(\pm p)| \rceil$. Assume that $q_\1\leq\frac{1}{2}$. Then, by constraint \eqref{eq:constraint} $q_\0 \geq \frac{1}{2}$ and $F$ is not symmetric. Contradiction. Hence, $q_\1>\frac{1}{2}$. By the same reasoning, $q_\0>\frac{1}{2}$).Two cases: 
\begin{itemize}
\item[i] $F$ is not $\maj$. Then, $q_\1>\frac{1}{2}+\frac{1}{2|N|}$ or $q_\0>\frac{1}{2}+\frac{1}{2|N|}$. Then $|\{\O\in\AB | F(\O)(p)= \1 \} \subset \{\O\in\AB | \maj(\O)(p)= \1 \}$ or $\{\O\in\AB | F(\O)(p)= \0 \} \subset \{\O\in\AB | \maj(\O)(p)= \0 \}$, therefore $\{\O\in\AB | F(\O)(p)= \ast \} \supset \{\O\in\AB | \maj(\O)(p)= \ast \}$. Therefore, $F$ does not minimize abstention. 

\item[ii] $F$ is $\maj$. Then, $\frac{1}{2}<q_\1,q_\0 \leq \frac{1}{2}+\frac{1}{2|N|}$. Assume that for some symmetric quota rule $F'$ with quotas $\lceil q'_\1 \times |\O(\pm p)| \rceil =  \lceil q'_\0 \times |\O(\pm p)| \rceil $: $|\{\O\in\AB | F'(\O)(p)= \ast \}| \leq |\{\O\in\AB \mid \maj(\O)(p)=\ast \}|$. Then, by the above reasoning, we know that $\frac{1}{2}<q'_\1,q'_\0\leq \frac{1}{2}+\frac{1}{2|N|}$, and $F'$ is $\maj$. Therefore, $F$ minimizes abstention.  
\end{itemize}
Hence, $F$ minimizes abstention iff $\frac{1}{2}<q_\1,q_\0 \leq \frac{1}{2}+\frac{1}{2|N|}$ iff $F$ is $\maj$.
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  proxy characterization

\begin{comment} HERE IS THE WHOLE THEOREM ADAPTED TO PROXY VERSION
\begin{theorem}\label{thm:quotarules}
Let $\S$ be a BA structure, let $F: (\AB_{c})^\N \to \AB$ be an aggregator and let $\pv_F = t\circ F$, with $t$ the abovedefined translation function. Then, the following three claims hold: 
\begin{enumerate}
\item $\pv_F$ is a proxy quota rule if and only if $F$ is anonymous, independent, monotonic, and responsive. 
\item $\pv_F$ is a symmetric proxy quota rule if and only if $F$ is an unbiased proxy quota rule. 
%IN THE OLD VERSION: WRONG (TRUE IN GENERAL, BUT NOT FOR A GIVEN N!) TO BE CORRECTED...
\item $\pv_F$ is the proxy majority rule $\pv_\maj$ if and only if $F$ is a symmetric proxy quota rule which minimizes collective abstention. %IN THE OLD VERSION: KINDA WRONG, FOR THE SAME REASON! TO BE CORRECTED.
\end{enumerate}
\end{theorem}
\end{comment}


